Improving the identification of antigenic sites in the H1N1 Influenza virus through accounting for the experimental structure in a sparse hierarchical Bayesian model

Understanding how genetic changes allow emerging virus strains to escape the protection afforded by vaccination is vital for the maintenance of effective vaccines. In the current work, we use structural and phylogenetic differences between pairs of virus strains to identify important antigenic sites on the surface of the influenza A(H1N1) virus through the prediction of haemagglutination inhibition (HI) assay, pairwise measures of the antigenic similarity of virus strains. We propose a sparse hierarchical Bayesian model that can deal with the pairwise structure and inherent experimental variability in the H1N1 data through the introduction of latent variables. The latent variables represent the underlying HI assay measurement of any given pair of virus strains and help account for the fact that for any HI assay measurement between the same pair of virus strains, the difference in the viral sequence remains the same. Through accurately representing the structure of the H1N1 data, the model is able to select virus sites which are antigenic, while its latent structure achieves the computational efficiency required to deal with large virus sequence data, as typically available for the influenza virus. In addition to the latent variable model, we also propose a new method, block integrated Widely Applicable Information Criterion (biWAIC), for selecting between competing models. We show how this allows us to effectively select the random effects when used with the proposed model and apply both methods to an A(H1N1) dataset.

==> RSSC_Further_Work.tex <==
\section{Further Work}

Further work involves investigating how different types of amino acid change at the same residue position on the structure affect antigenic variability. The data currently consists of indicators of amino acid change that are identical regardless of which particular amino acids are involved. However, given the range of biophysical properties among different amino acids, we expect the antigenic impact of a change to depend on both the location on the structure and the particular amino acids involved. In \cite{Reeve16} and \cite{Harvey16} variables were used that indicated a particular amino acid change at a given location. This will significantly increase the number of variables that must be selected from and therefore it is likely that the model will require additional information in order to prevent spurious results. Latent Gaussian processes can be used to include the additional information, e.g. \cite{Flippone13}, and will allow us to account for (a) differences in the antigenic impact of amino acid substitutions that depend on the amino acids involved and (b) similarities between changes of a certain type that occur at the same, or similar, locations on the protein surface.

%Further work involves investigating how different types of mutations affect antigenic variability. The data currently consists of indicators of mutational changes that occur regardless of the type of mutation. In \cite{Reeve16} and \cite{Harvey16} this was changed such that the variables indicated a particular type of mutation at a given location. This will significantly increase the number of variables that must be selected from and therefore it is likely that the model will require additional information in order to prevent spurious results. Latent Gaussian processes can be used to include the additional information, e.g. \cite{Flippone13}, and will allow us to introduce relationship between mutations of a certain type or mutations occurring at the same or similar locations.

%Finally, in order to use the eSABRE model on larger Influenza datasets with a larger number of pairs of reference and test strains, the method needs to be applied in a more computationally efficient manner. One way of doing this would be to split the datasets into $N$ different subsets and perform inference on those subsets. Recently \cite{NemethSherlock17} have demonstrated a novel way of recombining these sub-posteriors. They introduced Gaussian Process approximations for each sub-posterior density and then used these to create a tractable approximation to the full posterior. We can use this recombination method with the eSABRE model and this is relatively straightforward with our binary parameters of interest, $\bfgam$.
%
%What is less straight forward is specifying the priors for each of these data subsets, as each prior must be specified as its $N$th root. In the context of the work of \cite{NemethSherlock17} this is relatively straightforward, with the models used having relatively simple prior specifications. Specifying priors in this manner, however, becomes more complex in the context of Bayesian hierarchical models where not all the priors have fixed hyperparameters. To use the method of \cite{NemethSherlock17} in this context therefore requires a method for correcting the prior specification of the sub-posteriors.


\begin{algorithm}[b]
\SetAlgoLined
%\KwInput{Write here the result }
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
 \Input{Nominal hyperparameters $\hyperpt$}
 \Output{Corrected hyperparameters $\hyperp$}

 \While{prior $p(\param|\hyperp)$ is inconsistent with actual prior knowledge}{
  Chose a new nominal hyperparameter vector $\hyperpt$\;
  Run a multiple partition MCMC simulation without data\;
  %Obtain the posterior distribution $p(\param|\Data,\hyperpt)$ from (\ref{eq:Pmcmc})\;
  Compute the Kullback-Leibler divergence by application of (\ref{eq:KLE})\;
  Obtain new corrected hyperparameters $\hyperp$ by application of (\ref{eq:KLmin})\;
  %\eIf{condition}{
   %instructions1\;
   %}{
   %instructions2\;
  %}
 }
 \caption{Prior correction for combining sub-posteriors \label{algo:one}}
\end{algorithm}

If the data set $\Data$ is so large that the MCMC run time becomes onerous, the divide-and-conquer strategy of \cite{NemethSherlock17} can be applied, which is based on partitioning the data, $\Data = \{\Data_1,\Data_2,\ldots\Data_{\Npart}\}$, running $\Npart$ separate MCMC simulations in parallel to obtain the sub-posterior  
distributions $p(\param|\Data_i)$, $i=1,\ldots,\Npart$, 
and then combining these sub-posteriors along the following lines:
\begin{equation}
\label{eq:Pmcmc}
p(\param|\Data,\hyperp) \propto p(\Data|\param)p(\param|\hyperp) 
\; = \;
\prod_{i=1}^{\Npart} \Big(p(\Data_i|\param) q(\param|\hyperp)\Big)
\;\propto \;
\prod_{i=1}^K p(\param|\Data_i,\hyperp)
\end{equation}
where
\begin{equation}
q(\param|\hyperp) \; \propto \; 
\sqrt[\Npart]{p(\param|\hyperp)}
\end{equation}
 The practical difficulty in applying this scheme to a complex hierarchical Bayesian model as proposed in our work is 
 the intractability of the prior distribution $q(\param|\hyperp)$. Ideally, we would like to find hyperparameters $\hyperpt$ so that $q(\param|\hyperpt)$ matches as closely as possible the original prior $p(\param|\hyperp)$, e.g. by minimising the Kullback-Leibler divergence
\begin{equation}
\KLE(\hyperp,\hyperpt)
\; = \; 
\int q(\param|\hyperpt) \log\left(\frac{q(\param|\hyperpt)}{p(\param|\hyperp)} \right) d\param
\end{equation}
This is infeasible, due to the intractability of  $E(\hyperp,\hyperpt)$ as a function of $\hyperpt$. However, what we can do instead is minimise 
$\KLE(\hyperp,\hyperpt)$ for fixed $\hyperpt$ with respect to $\hyperp$, since
\begin{eqnarray}
\KLE(\hyperp,\hyperpt)
& = &
- \int q(\param|\hyperpt) \log\Big(p(\param|\hyperp)\Big) d\param
\,+\, C_{\hyperpt}
\\
& \approx & 
- \sum_{i=1}^N
\log\Big(p(\param_i|\hyperp)\Big)
\,+\, C_{\hyperpt}
\label{eq:KLE}
\end{eqnarray}
where $C_{\hyperpt}$ is a constant with respect to $\hyperp$, and 
$\{\param_i\}_{i=1}^{N}$ is a sample from the distribution $q(\param|\hyperpt)$, which is 
straightforwardly obtained by running the parallel multi-partition MCMC algorithm of \cite{NemethSherlock17} without data.
So while we cannot specify the modified prior distribution $q(\param|\hyperpt)$ directly, we can find the original prior distribution $p(\param|\hyperp)$
that provides the closest match:
\begin{equation}
\mathrm{argmin}_{\hyperp} \KLE(\hyperp,\hyperpt)
\label{eq:KLmin}
\end{equation}
If that prior distribution is unacceptable, due to insufficient agreement with the actual prior knowledge, a new hyperparameter vector $\hyperpt$ can be tried until the agreement  is acceptable.   A pseudo code representation of the algorithm is shown in Algorithm~\ref{algo:one}.
Note that MCMC simulations without data correspond to the extreme annealing end of a parallel tempering scheme, where convergence and mixing are usually fast, and the computational costs are thus comparatively low. Also, the prior distribution is usually chosen to be vague due to lack of actual prior knowledge. In that case, the condition in the {\tt While} statement on line 1 of the algorithm can be replaced by the following less stringent criterion: {\tt While $p(\param|\hyperp)$ is insufficiently disperse}.

\begin{figure}[tb]
\centering
\includegraphics[scale=0.3]{figCostanza1.png}
\includegraphics[scale=0.3]{figCostanza2.png}
\caption
{
\label{fig:subMCMC}
{\bf ROC curves for assessment of the sub-posterior method.}
The blue lines show the ROC curve for the proper posterior distribution, obtained by running an MCMC simulation on the whole data set. The thin  black lines show the ROC curves of the sub-posterior distributions, obtained by running ten MCMC simulations in parallel on ten non-overlapping subsets of the data, each containing a tenth of the total data. The red lines show the ROC curves obtained by combining the posterior distributions according to (\ref{eq:Pmcmc}). Left panel: no adjustment of the hyperparameters. Right: adjustment of the hyperparameters, as discussed in the text. The improvement in the agreement between the two curves is clearly noticeable. The simulations were carried out by Costanza Calzolari as part of her Bachelor's project at the University of Glasgow, supervised by the authors.
}
\end{figure}

We have carried out a simple proof of concept study on simulated data, similar to those described in Section~6, where we have compared the performance of the sub-posterior method with standard MCMC. The data were partitioned into 10 non-overlapping subsets, each containing a tenth of the original data. Ten MCMC simulations were run in parallel, and the sub-posterior were then combined, based on (\ref{eq:Pmcmc}), as described in \cite{NemethSherlock17}. These results were compared with a standard MCMC simulation on the complete data set. The results are shown in Figure~\ref{fig:subMCMC} and suggest that when correcting for the mismatch between the hyperparameters, a similar performance can be achieved as with standard MCMC, but at substantially reduced computational costs.

A more extensive exploration is beyond the remit of the present paper, but will provide an interesting topic for future research.
